Learning with Logical Constraints but without Shortcut Satisfaction

Recent studies in neuro-symbolic learning have explored the integration of logical knowledge into deep learning via encoding logical constraints as an additional loss function. However, existing approaches tend to vacuously satisfy logical constraints through shortcuts, failing to fully exploit the knowledge. In this paper, we present a new framework for learning with logical constraints. Specifically, we address the shortcut satisfaction issue by introducing dual variables for logical connectives, encoding how the constraint is satisfied. We further propose a variational framework where the encoded logical constraint is expressed as a distributional loss that is compatible with the model's original training loss. The theoretical analysis shows that the proposed approach bears salient properties, and the experimental evaluations demonstrate its superior performance in both model generalizability and constraint satisfaction.

==> tables/table_hwf.tex <==
\eat{% this is the results of weight_decay = 5e-4...
\begin{table}[t]
\centering
\caption{Results on HWF dataset.}
%\resizebox{1\columnwidth}{!}{
\begin{tabular}{crrrr}
  \toprule
  \multirow{2}{*}{Method} & \multicolumn{2}{c}{Calculation (\%)} & \multicolumn{2}{c}{Constraint  (\%)}\\
   \cmidrule(lr){2-3}\cmidrule(lr){4-5} & 2/80$^*$ & 5/20$^*$ & 2/80$^*$ & 5/20$^*$ \\  
  \midrule
    Baseline & 57.4 & 75.6 & 64.0 & 81.5 \\
    PD$_1$ & 62.1 & 76.5 & 63.2 & 78.6 \\
    PD$_2$ & 62.5 & 76.4 & 62.5 & 78.4 \\    
    DL2 & 62.9 & 79.3 & 57.5 & 86.6 \\  
    \midrule
    Ours & 65.1 & 79.5 & 82.4 & 92.8 \\
  \bottomrule
\end{tabular}
%}
 \begin{tablenotes}
        \footnotesize
        \item[1]*  It refers to the proportion of labeled and unlabeled data used from the training set. 
 \end{tablenotes}
\label{tab:hwf-res}
\end{table}
}

% this is the results of weight_decay = 5e-4...

{\small
\begin{table}[t]
\centering
\caption{Results of the handwritten formula recognition task. The proposed approach outperforms the competitors in both calculation accuracy and logical constraint satisfaction.}
%\resizebox{1\columnwidth}{!}{
%\vspace{1ex}
\begin{tabular}{crrrr}
  \toprule
  \multirow{2}{*}{Method} & \multicolumn{2}{c}{2/80$^*$ Data Split} & \multicolumn{2}{c}{5/20$^*$ Data Split}\\
   \cmidrule(lr){2-3}\cmidrule(lr){4-5} & Acc. (\%) & Sat. (\%) & Acc. (\%) & Sat. (\%) \\  
  \midrule
    Baseline & 57.4 & 64.0 & 75.6 & 81.5 \\
    PD$_1$ & 62.1 & 63.2 & 76.5 & 78.6 \\
    PD$_2$ & 62.5 & 62.5 & 76.4 & 78.4 \\    
    DL2 & 62.9 & 57.5 & 79.3 & 86.6 \\  
    \midrule
    Ours & {\bf 65.1} & {\bf 82.4} & {\bf 79.5} & {\bf 92.8} \\
  \bottomrule
\end{tabular}
%}
 \begin{tablenotes}
        \footnotesize
        \item[1]*  It refers to the proportion of labeled and unlabeled data used from the training set. 
 \end{tablenotes}
\label{tab:hwf-res}
\end{table}
}

==> tables/table_srp.tex <==
% this is the results of weight_decay = 5e-4...
{\small
\begin{table}[t]
\centering
\caption{Results on the shortest distance prediction task. The proposed approach outperforms the competitors in both prediction accuracy and constraint satisfaction.}
%\vspace{1ex}
%\resizebox{1\columnwidth}{!}{
\begin{tabular}{crr}
  \toprule
  Method & {MSE / MAE} & Constraint Sat. (\%) \\
  \midrule
    Baseline & 8.90 / 2.07 & 43.9 \\
    PD$_2$ & 9.11 / 2.11 & 46.1 \\
    DL2 & 14.21 / 2.68 & 65.3 \\  
    \midrule
    Ours & {\bf 7.09 / 1.87} & {\bf 69.0} \\
  \bottomrule
\end{tabular}
%}
\label{tab:srp-res}
\end{table}
}
